Reconstructing veriT Proofs in Isabelle/HOL

Automated theorem provers are now commonly used within interactive theorem provers to discharge an increasingly large number of proof obligations. To maintain the trustworthiness of a proof, the automatically found proof must be verified inside the proof assistant. We present here a reconstruction procedure in the proof assistant Isabelle/HOL for proofs generated by the satisfiability modulo theories solver veriT which is part of the smt tactic. We describe in detail the architecture of our improved reconstruction method and the challenges we faced in designing it. Our experiments show that the veriT-powered smt tactic is regularly suggested by Sledgehammer as the fastest method to automatically solve proof goals.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{Haniel Barbosa and Giselle Reis (Eds.): Sixth Workshop\\ on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 301, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.301.6}{10.4204/EPTCS.301.6}}
\pdfoutput=1

